Improving Image Restoration by Revisiting Global Information Aggregation

Global operations, such as global average pooling, are widely used in top-performance image restorers. They aggregate global information from input features along entire spatial dimensions but behave differently during training and inference in image restoration tasks: they are based on different regions, namely the cropped patches (from images) and the full-resolution images. This paper revisits global information aggregation and finds that the image-based features during inference have a different distribution than the patch-based features during training. This train-test inconsistency negatively impacts the performance of models, which is severely overlooked by previous works. To reduce the inconsistency and improve test-time performance, we propose a simple method called Test-time Local Converter (TLC). Our TLC converts global operations to local ones only during inference so that they aggregate features within local spatial regions rather than the entire large images. The proposed method can be applied to various global modules (e.g., normalization, channel and spatial attention) with negligible costs. Without the need for any fine-tuning, TLC improves state-of-the-art results on several image restoration tasks, including single-image motion deblurring, video deblurring, defocus deblurring, and image denoising. In particular, with TLC, our Restormer-Local improves the state-of-the-art result in single image deblurring from 32.92 dB to 33.57 dB on GoPro dataset. The code is available at https://github.com/megvii-research/tlc.

==> tabs/Fig_distribution.tex <==
% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{imgs/MPRNet_module.stage2_encoder.encoder_level1.0.CA.avg_pool.pdf}
% % \includegraphics[width=0.58\linewidth]{imgs/HINet_module.down_path_2.3.norm.avgpool.pdf}
% \caption{
% Visualization of the statistics (mean) distribution of the first SE layer of the second encoder in MPRNet on GoPro dataset.
% Green: the distribution when training with patches; Blue: the distribution when testing with images; Red: the distribution when testing with images and TLSC is adopted (denoted as MPRNet-local).
% (a) The original test scheme results in distribution shifts.
% (b) Distribution shifts could be reduced by our proposed TLSC.
% }
% \label{fig:distribution}
% \end{figure}


\begin{figure}[t!]
    \centering
    \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,center}}}]{figure}[\FBwidth]{
    \caption{
Visualization of the statistics (mean) distribution of the first SE layer of the second encoder in MPRNet on GoPro dataset.
% Green: the distribution when training with patches; Blue: the distribution when testing with images; Red: the distribution when testing with images and TLSC is adopted (denoted as MPRNet-local).
(a) The inconsistency between training (w/ patches) and testing (w/ full images) results in distribution shifts.
(b) Distribution shifts could be reduced when our proposed TLSC is adopted (denoted as MPRNet-local).
}
\label{fig:distribution}
}{\includegraphics[height=100px]{imgs/MPRNet_module.stage2_encoder.encoder_level1.0.CA.avg_pool.pdf}}
\end{figure}

==> tabs/Fig_sota.tex <==
\begin{figure}[t]
\begin{center}
 \includegraphics[width=\linewidth]{imgs/sota3.pdf}  
\end{center}
    \caption{Improvements of applying TLSC to public available trained models (\ie MPRNet~\cite{zamir2021multi}, SPDNet~\cite{fang2020multi} and FFANet~\cite{qin2020ffa}) on three image restoration tasks (\ie GoPro~\cite{nah2017deep} for deblurring, SPA-Data~\cite{wang2019spatial} for deraining and SOTS~\cite{li2018benchmarking} for dehazing). 
    Clearly, our approach not only improve all models without re-training, but exceeds the previous best results (ploted as green dashed line) on deburring~\cite{chen2021hinet} and deraining~\cite{fang2020multi} tasks.
    }
    \label{fig:SOTA}
\end{figure}
